Creating small circular, elliptical, and triangular droplets of quark-gluon plasma

The experimental study of the collisions of heavy nuclei at relativistic energies has established the properties of the quark-gluon plasma (QGP), a state of hot, dense nuclear matter in which quarks and gluons are not bound into hadrons. In this state, matter behaves as a nearly inviscid fluid that efficiently translates initial spatial anisotropies into correlated momentum anisotropies among the produced particles, producing a common velocity field pattern known as collective flow. In recent years, comparable momentum anisotropies have been measured in small-system proton-proton ($p$$+$$p$) and proton-nucleus ($p$$+$$A$) collisions, despite expectations that the volume and lifetime of the medium produced would be too small to form a QGP. Here, we report on the observation of elliptic and triangular flow patterns of charged particles produced in proton-gold ($p$$+$Au), deuteron-gold ($d$$+$Au), and helium-gold ($^3$He$+$Au) collisions at a nucleon-nucleon center-of-mass energy $\sqrt{s_{_{NN}}}$~=~200 GeV. The unique combination of three distinct initial geometries and two flow patterns provides unprecedented model discrimination. Hydrodynamical models, which include the formation of a short-lived QGP droplet, provide a simultaneous description of these measurements.

==> Makefile <==
SRC = main.tex main.bib natphys.tex methods.tex

all: main methods natphys

# Simple case:  no figures or BibTeX
main.pdf: $(SRC)
	pdflatex main
	pdflatex main
	pdflatex main

# If all figures are PDF'd, then we can use pdflatex instead
# (This requires changing the [dvips] driver to [pdftex]
# on the \usepackage{graphics} line in main.tex.)
main:
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main

methods:
	pdflatex methods
	bibtex methods
	pdflatex methods
	pdflatex methods

natphys:
	pdflatex natphys

distclean:
	-@rm *.{aux,toc,dvi,lof,lot,log,lom,bbl,blg,pdf,ps,out} *~

